Chance-Constrained Optimization in Contact-Rich Systems for Robust Manipulation

This paper presents a chance-constrained formulation for robust trajectory optimization during manipulation. In particular, we present a chance-constrained optimization for Stochastic Discrete-time Linear Complementarity Systems (SDLCS). To solve the optimization problem, we formulate Mixed-Integer Quadratic Programming with Chance Constraints (MIQPCC). In our formulation, we explicitly consider joint chance constraints for complementarity as well as states to capture the stochastic evolution of dynamics. We evaluate robustness of our optimized trajectories in simulation on several systems. The proposed approach outperforms some recent approaches for robust trajectory optimization for SDLCS.

==> problemform.tex <==
\section{Problem Description}\label{sec:prob_formulation}
In this section, we describe a robust trajectory optimization problem for dynamical systems with frictional interaction. We describe several sources of uncertainty and how they can be potentially modeled to be used in robust optimization. To present a concrete example and for clarity of exposition, we explain a planar pushing example and explain different uncertainties in the pusher-slider system.

